Scalar fields on fluctuating hyperbolic geometries

We present results on the behavior of the boundary-boundary correlation function of scalar fields propagating on discrete two-dimensional random triangulations representing manifolds with the topology of a disk. We use a gravitational action that includes a curvature squared operator, which favors a regular tessellation of hyperbolic space for large values of its coupling. We probe the resultant geometry by analyzing the propagator of a massive scalar field and show that the conformal behavior seen in the uniform hyperbolic space survives as the coupling approaches zero. The analysis of the boundary correlator suggests that holographic predictions survive, at least, weak quantum gravity corrections. We then show how such an $R^2$ operator might be induced as a result of integrating out massive lattice fermions and show preliminary result for boundary correlation functions that include the effects of this fermionic backreaction on the geometry.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
%\usepackage{subfig}
%\usepackage{caption}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{pinlabel, color}
\usepackage{multirow}
% \usepackage[hyperindex, pdftex,colorlinks=true,
%                       pdfstartview=FitV,
%                       linkcolor=blue,
%                       citecolor=blue,
%                       urlcolor=blue,
%           ]{hyperref}
\usepackage{array}
% \usepackage[section]{placeins}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\arccosh}{{\rm arccosh}}
